Appearance Pointers -- Multimodal Region Control of Diffusion Transformers

Controllable image generation remains challenging for creative professionals, who often require precise regional control over materials, object identities, and spatial arrangements that cannot be reliably achieved through text prompting alone. Diffusion Transformers (DiTs) can natively ingest heterogeneous tokens stemming from texts and images, but they lack mechanisms for determining where and how these tokens should influence the output. We introduce appearance pointers, compact tokens that guide DiTs toward the correct appearance cues at the correct spatial locations by aligning text or image inputs with user-specified masks. Appearance pointers are produced by a region correspondence network and refined through a spatial aggregation mechanism, enabling the model to handle multiple regional descriptions without significantly increasing token load. Our approach introduces the first modality-agnostic interface for localized multimodal control in a DiT without retraining the base model from scratch. Across a range of metrics, our single model reaches or surpasses the performance of modality-specific state of the art methods, offering a simple and extensible path toward precise, region-aware, multimodal guidance in generative image synthesis.

==> latexmkrc <==
#!/usr/bin/perl

#--------------------
# Configurable choices for compilation of external documents

# Subdirectory for output files from compilation of external documents:
$sub_doc_output = 'output-subdoc';

# Options to supply to latexmk for compilation of external documents:
@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

#--------------------

# Add a pattern for xr's log-file message about missing files to latexmk's
# list.  Latexmk's variable @file_not_found is not yet documented.
# This line isn't necessary for v. 4.80 or later of latexmk.
push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne '') && ($sub_doc_output ne '.') ) {
               # In this case, .aux file generated by pdflatex isn't in same
               # directory as the .tex file.
               # Therefore:
               # 1. Actual generated aux file must be listed as produced by this
               #    rule, so that latexmk deals with dependencies correctly.
               #    (Problem to overcome: If $sub_dir_output is same as $aux_dir
               #    for the main document, xr may read the .aux file in the
               #    aux_dir rather than the one the cus dep is assumed by latexmk
               #    to produce, which is in the same directory as the .tex source
               #    file for this custom dependency.)
               #    Use not-yet-documented latexmk subroutine rdb_add_generated
               #    to do this:
               # 2. A copy of the .aux file must be in same directory as .tex file
               #    to satisfy latexmk's definition of a custom dependency.
             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}



## Put this (Perl) file in the root of your Overleaf project. It overrides the
## `pdflatex` compilation command to run GhostScript as a post-process which will
## compress non-JPEG images to JPEG in the output PDF file. The JPEG quality
## settings are set to high to minimize the loss of image quality. This should
## work well even for images that contain a lot of high-frequency noise.
## To disable, simply rename the file to something other than latexmkrc.
##
## Created by Iliyan Georgiev.

## Quality settings
$PDF_VERSION = 1.4;
$IMG_DOWNSAMPLE = 'true';
$IMG_DOWNSAMPLE_DPI = 600;
$IMG_DOWNSAMPLE_THRESHOLD = 1.0;
$IMG_COMPRESSION_QFACTOR = 0.2;  # lower is better (try 0.08 for higher quality)
$PASSTHROUGH_JPEGS = 'true';

## Don't modify these, they are specified by Overleaf
$GS_INPUT_FILE = '%B.pdf';
$GS_OUTPUT_FILE = '%B-embed.pdf';

## You can try setting below: -dNEWPDF=true
## This fails in the current GhostScript v9.55 on Overleaf 
$GS_COMMAND = "gs
   -sDEVICE=pdfwrite
   -sOutputFile=$GS_OUTPUT_FILE
   -dCompatibilityLevel=$PDF_VERSION
   -dPDFSETTINGS=/default
   -dFastWebView=true
   -dEmbedAllFonts=true
   -dSubsetFonts=true
   -dCompressFonts=true
   -dDetectDuplicateImages=true
   -dDoThumbnails=false
   -dAutoRotatePages=/None
   -dDownsampleColorImages=$IMG_DOWNSAMPLE
   -dColorImageDownsampleType=/Bicubic
   -dColorImageDownsampleThreshold=$IMG_DOWNSAMPLE_THRESHOLD
   -dColorImageResolution=$IMG_DOWNSAMPLE_DPI
   -dDownsampleGrayImages=$IMG_DOWNSAMPLE
   -dGrayImageDownsampleType=/Bicubic
   -dGrayImageDownsampleThreshold=$IMG_DOWNSAMPLE_THRESHOLD
   -dGrayImageResolution=$IMG_DOWNSAMPLE_DPI
   -dDownsampleMonoImages=$IMG_DOWNSAMPLE
   -dMonoImageDownsampleType=/Subsample
   -dMonoImageDownsampleThreshold=$IMG_DOWNSAMPLE_THRESHOLD
   -dMonoImageResolution=$IMG_DOWNSAMPLE_DPI
   -dConvertCMYKImagesToRGB=true
   -dColorImageFilter=/DCTEncode
   -dGrayImageFilter=/DCTEncode
   -dMonoImageFilter=/CCITTFaxEncode
   -dColorConversionStrategy=/LeaveColorUnchanged
   -dPassThroughJPEGImages=$PASSTHROUGH_JPEGS
   -dProcessColorModel=/DeviceRGB
   -dRenderIntent=1
   -dDefaultRenderingIntent=/Perceptual
   -dUseArtBox
   -dNEWPDF=false
   -dNOPAUSE
   -dBATCH
   -c \"<< /ColorACSImageDict << /VSamples [ 1 1 1 1 ] /HSamples [ 1 1 1 1 ] /QFactor $IMG_COMPRESSION_QFACTOR /Blend 1 /ColorTransform 1 >> >> setdistillerparams\"
   -f $GS_INPUT_FILE";

## Remove new-line characters from GhostScript command
$GS_COMMAND =~ s/\n//g;

## Set the pdflatex command to be used by Overleaf
$pdflatex = "pdflatex %O %S; $GS_COMMAND; mv %B-embed.pdf %B.pdf";

## For debugging
# print "$GS_COMMAND\n";
# print "$pdflatex\n";


==> sec/03_background.tex <==
\section{Preliminaries}





% \paragraph{Flow Matching} 



% \paragraph{Positional Encoding with RoPE:}
% \paragraph{Dual Transformer:}
% \paragraph{Single Transformer:}

% \rahul{
% \begin{enumerate}
%     \item Detail Flux Arch. with the single and dual attention blocks
%     \item processing/embedding text and image features by embedder
%     \item Some brief details about the Rope and position embedding mechanism as well
% \end{enumerate}
% }

==> sec/Z_CVPR_template.tex <==

\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets the figure captions and references in a smaller font.
The reason why such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The review process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in 11 pages.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler that should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use the options of \texttt{cvpr.sty} to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Use fractional references (\eg, this line is $087.5$), although in most cases the approximate location would be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please, number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for the reader to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean that some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not mean that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper, we present a performance analysis of our previous paper [1], and show that it is inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper, we present a performance analysis of the paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time that covers similar or overlapping material, you may need to refer to that submission to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, do not assume that the reviewers will read this material.

Sometimes your paper is about a problem that you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think that it is likely that the new article was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
However, for your results, you should not identify yourself and should not mention your participation in the challenge.
Instead, present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison with other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has only two authors.

\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}



\section{Formatting your paper}
\label{sec:formatting}

All text must be in two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
The columns should be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered, and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

The captions of the figures and tables should be in 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centered.  Table captions should be above tables, while figure captions should be below figures.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period, and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use the footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example, at the beginning of the sentence, you can use
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, include the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When citing multiple papers at once, make sure that you cite them in numerical order such as this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \caption{Results.   Ours is better.}
  \label{tab:example}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead, use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise and, therefore, must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it is almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence, avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.


\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/eccv_template.tex <==

\begin{abstract}
  The abstract should concisely summarize the contents of the paper. 
  While there is no fixed length restriction for the abstract, it is recommended to limit your abstract to approximately 150 words.
  Please include keywords as in the example below. 
  This is required for papers in LNCS proceedings.
  \keywords{First keyword \and Second keyword \and Third keyword}
\end{abstract}

\section{Introduction}
\label{sec:intro}

This document serves as an example submission to ECCV \ECCVyear{}.
It illustrates the format authors must follow when submitting a paper. 
At the same time, it gives details on various aspects of paper submission, including preservation of anonymity and how to deal with dual submissions.
We advise authors to read this document carefully.

The document is based on Springer LNCS instructions as well as on ECCV policies, as established over the years.

\section{Initial Submission}

\subsection{Language}
All manuscripts must be in English.


\subsection{Template}
Papers must be prepared with the official LNCS style from Springer.
This applies to both review and camera-ready versions.
Springer requires manuscripts to be prepared in \LaTeX{} (strongly encouraged) or Microsoft Word. 

Authors preparing their paper with \LaTeX{} must use the template provided by ECCV, which is based on the corresponding Springer class file \texttt{llncs.cls} but includes line numbers for review (\cref{sec:line-numbering}) and properly anonymizes the paper for review (as in this example document).
Authors who -- for whatever reason -- cannot use \LaTeX{} can alternatively use the official LNCS Word template from Springer.
However, it is the authors' responsibility to ensure that the resulting PDF file is consistent with this example paper and follows it as closely as possible (\ie, includes line numbers, is properly anonymized, \etc).

We would like to stress that the class/style files and the template must not be manipulated and that the guidelines regarding font sizes and format must be adhered to. 
For example, please refrain from using any \LaTeX{} or \TeX{} command that modifies the layout settings of the template (\eg, \verb+\textheight+, \verb+\vspace+, \verb+\baselinestretch+, \etc).
Such manual layout adjustments should be limited to very exceptional cases.
This is to ensure that the end product is as homogeneous as possible.

Papers that differ significantly from the required style may be rejected without review.


\subsubsection{Fonts.}
Springer's templates for \LaTeX{} are based on CMR, and the XML templates for Word are based on Times. 
We ask you to use the font according to the template used for your papers. 
Specifically, please refrain from using Times when preparing your paper with \LaTeX{}.
Using a different font can be interpreted as purposely circumventing the length limitations and may lead to rejection without review.


\subsection{Paper Length}
Papers submitted for review must be complete. 
The length should match that intended for final publication. 
Papers accepted for the conference will be allocated 14 pages (plus additional pages for references) in the proceedings. 
Note that the allocated 14 pages do not include the references. 
The reason for this policy is that we do not want authors to omit references for sake of space limitations.

Papers with more than 14 pages (excluding references) will be rejected without review.
This includes papers where the margins and formatting including the font are deemed to have been significantly altered from those laid down by this style guide.

The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts. 
The reviewing process cannot determine the suitability of the paper for presentation in 14 pages if it is reviewed in 16.


\subsection{Paper ID}
It is imperative that the paper ID is mentioned on each page of the manuscript of the review version.
Enter your paper ID in the appropriate place in the \LaTeX{} template (see \texttt{\%TODO REVIEW}).
The paper ID is a number automatically assigned to your submission when registering your paper submission on the submission site.


\subsection{Line Numbering}
\label{sec:line-numbering}
All lines should be numbered in the initial submission, as in this example document. 
This makes reviewing more efficient, because reviewers can refer to a line on a page. 
Line numbering is removed in the camera-ready version.


\section{Policies}
The policies governing the review process of ECCV \ECCVyear{} are detailed on the conference webpage (see \url{ https://eccv.ecva.net/Conferences/2026/SubmissionPolicies}), such as regarding confidentiality, dual submissions, double-blind reviewing, plagiarism, and more. 
By submitting a paper to ECCV, the authors acknowledge that they have read the submission policies and that the submission follows the rules set forth.

Accepted papers will be published in LNCS proceedings with Springer.
To that end, authors must follow the Springer Nature Code of Conduct for Authors (see \url{https://www.springernature.com/gp/authors/book-authors-code-of-conduct}).
We would like to draw particular attention to the policies regarding figures and illustrations, as well as ethical approval and informed consent, which are also reproduced on the ECCV website.


\section{Preserving Anonymity}
\label{sec:blind}
ECCV reviewing is double blind, in that authors do not know the names of the area chair/reviewers of their papers, and the area chairs/reviewers cannot, beyond reasonable doubt, infer the names of the authors from the submission and the additional material. 
You must not identify the authors nor provide links to websites that identify the authors, neither in the paper nor in the supplemental material.
If you need to cite a different paper of yours that is being submitted concurrently to ECCV, you should \emph{(1)} cite these papers anonymously, \emph{(2)} argue in the body of your paper why your ECCV paper is non-trivially different from these concurrent submissions, and \emph{(3)} include anonymized versions of those papers in the supplemental material.
Violation of any of these guidelines may lead to rejection without review. 

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
  \begin{center}
      An analysis of the frobnicatable foo filter.
  \end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}

An example of an acceptable paper:
\begin{quote}
  \begin{center}
     An analysis of the frobnicatable foo filter.
  \end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission [1] as supplemental material and cite it as
\begin{quote}
  [1] Authors. ``The frobnicatable foo filter'', ECCV \ECCVyear Submission ID 00324, Supplied as supplemental material {\tt 00324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not \emph{require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Anonymous24b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem, which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the ECCV audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.

For sake of anonymity, authors must omit acknowledgements in the review copy. 
They can be added later when you prepare the final copy.


\section{Formatting Guidelines}

\subsection{Headings}
Headings should be capitalized (\ie, nouns, verbs, and all other words except articles, prepositions, and conjunctions should be set with an initial capital) and should, with the exception of the title, be aligned to the left.
Only the first two levels of section headings should be numbered, as shown in \cref{tab:headings}.
The respective font sizes are also given in \cref{tab:headings}. 
Kindly refrain from using ``0'' when numbering your section headings.
Words joined by a hyphen are subject to a special rule. 
If the first word can stand alone, the second word should be capitalized.

\begin{table}[tb]
  \caption{Font sizes of headings. 
    Table captions should always be positioned \emph{above} the tables.
  }
  \label{tab:headings}
  \centering
  \begin{tabular}{@{}lll@{}}
    \toprule
    Heading level & Example & Font size and style\\
    \midrule
    Title (centered)  & {\Large\bf Lecture Notes \dots} & 14 point, bold\\
    1st-level heading & {\large\bf 1 Introduction} & 12 point, bold\\
    2nd-level heading & {\bf 2.1 Printing Area} & 10 point, bold\\
    3rd-level heading & {\bf Headings.} Text follows \dots & 10 point, bold\\
    4th-level heading & {\it Remark.} Text follows \dots & 10 point, italic\\
  \bottomrule
  \end{tabular}
\end{table}

Here are some examples of headings: 
``Criteria to Disprove Context-Freeness of Collage Languages'', ``On Correcting the Intrusion of Tracing Non-deterministic Programs by Software'', ``A User-Friendly and Extendable Data Distribution System'', ``Multi-flip Networks: Parallelizing GenSAT'', ``Self-determinations of Man''.


\subsection{Figures}
\label{sect:figures}
For \LaTeX{} users, we recommend integrating figures in your paper using the package \texttt{graphicx}.

It is essential that all illustrations are clear and legible. 
Vector graphics (rather than rasterized images) should be used for diagrams and schemas whenever possible. 
Please check that the lines in line drawings are not interrupted and have a constant width. 
Line drawings are to have a resolution of at least 800 dpi (preferably 1200 dpi).
Grids and details within figures must be clearly legible and may not be written one on top of the other. 
The lettering in figures should not use font sizes smaller than 6\:pt ($\sim$2\:mm character height). 

Figures should be numbered and should have a caption, which should always be positioned \emph{under} the figures, in contrast to the caption belonging to a table, which should always appear \emph{above} the table.
Figures and Tables should be cross-referred in the text.

If they are short, they are centered between the margins (\cf \cref{fig:short}). 
Longer captions, covering more than one line, are justified (\cref{fig:example} shows an example). 
Captions that do not constitute a full sentence, do not have a period.


\begin{figure}[tb]
  \centering
  \includegraphics[height=6.5cm]{eijkel2}
  \caption{One kernel at $x_s$ (\emph{dotted kernel}) or two kernels at $x_i$ and $x_j$ (\emph{left and right}) lead to the same summed estimate at $x_s$.
    This shows a figure consisting of different types of lines.
    Elements of the figure described in the caption should be set in italics, in parentheses, as shown in this sample caption. 
    The last sentence of a figure caption should generally end with a full stop, except when the caption is not a full sentence.
  }
  \label{fig:example}
\end{figure}

\begin{figure}[tb]
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Centered, short example caption}
  \label{fig:short}
\end{figure}

If possible (\eg, if you use \LaTeX) please define figures as floating objects. 
\LaTeX{} users, please avoid using the location parameter ``h'' for ``here''. 
If you have to insert a pagebreak before a figure, please ensure that the previous page is completely filled.


\subsection{Formulas}
Displayed equations or formulas are centered and set on a separate line (with an extra line or half line space above and below). 
Equations should be numbered for reference. 
The numbers should be consecutive within the contribution, with numbers enclosed in parentheses and set on the right margin.
For example,
\begin{align}
  \psi (u) & = \int_{0}^{T} \left[\frac{1}{2}
  \left(\Lambda_{0}^{-1} u,u\right) + N^{\ast} (-u)\right] \text{d}t \; \\
& = 0
\end{align}
and 
\begin{equation}
  E = m\cdot c^2.
  \label{eq:important}
\end{equation}
Please do not include section counters in the numbering.

Numbering equations makes reviewing more efficient, because reviewers can refer to a line on a page.  
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{https://doi.org/10.1063/1.2811173}.

% No color equations in Springer publications.
Equations should never be in color and should be punctuated in the same way as ordinary text.
They should not be pasted in as figures.


\subsubsection{Lemmas, Propositions, and Theorems.}
The numbers accorded to lemmas, propositions, and theorems, \etc should appear in consecutive order, starting with Lemma 1. 
Please do not include section counters in the numbering like ``Theorem 1.1''.


\subsection{Footnotes.}
The superscript numeral used to refer to a footnote appears in the text either directly after the word to be discussed or -- in relation to a phrase or a sentence -- following the punctuation mark (comma, semicolon, or period).%
\footnote{The footnote numeral is set flush left and the text follows with the usual word spacing. 
  Second and subsequent lines are indented. 
}
For remarks pertaining to the title or the authors' names, in the header of a paper, symbols should be used instead of a number.
Please note that no footnotes may be included in the abstract.


\subsection{Cross References}
For the benefit of author(s) and readers, please use the
\begin{verbatim}
  \cref{...}
\end{verbatim}
command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:example} and \cref{tab:headings}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:example,fig:short-a}.
  You may also return to \cref{sec:intro} or look at \cref{eq:important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
\begin{verbatim}
  \Cref{...}
\end{verbatim}
command. Here is an example:
\begin{quotation}
  \Cref{fig:example} is also quite important.
\end{quotation}


\subsection{Program Code}
Program listings or program commands in the text are normally set in typewriter font (\eg, \texttt{printf("Hello world!\textbackslash{}n");}).


\subsection{Citations}
Arabic numbers are used for citation, which is sequential either by order of citation or by alphabetical order of the references, depending on which sequence is used in the list of references. 
The reference numbers are given in brackets and are not superscript.
Please observe the following guidelines:
\begin{itemize}
\item Single citation: \cite{Anonymous24}
\item Multiple citation: \cite{Alpher02,Alpher03,Alpher05,Anonymous24b,Anonymous24}. 
  The numbers should be listed in numerical order.
  If you use the template as advised, this will be taken care of automatically.
\item If an author's name is used in the text: Alpher \cite{Alpher02} was the first \ldots
\end{itemize}
Please write all references using the Latin alphabet. If the title of the book you are referring to is, \eg, in Russian or Chinese, then please write (in Russian) or (in Chinese) at the end of the transcript or translation of the title.
All references cited in the text should be in the list of references and vice versa.

References should be formatted with the official LNCS reference style.
The \LaTeX{} template already takes care of that through the use of the \texttt{splncs04.bst} Bib\TeX{} style file.
Springer strongly encourages you to include DOIs (Digital Object Identifiers) in your references (\cf \cite{ECCV2022}). 
The DOI is a unique code allotted by the publisher to each online paper or journal article. 
It provides a stable way of finding published papers and their metadata. 
The insertion of DOIs increases the overall length of the references section, but this should not concern you as the reference section is not counted toward the page limit.


\subsection{Miscellaneous}
Compare the following:
\begin{center}
  \begin{tabular}{ll}
    \verb'$conf_a$'          & $\qquad conf_a$ \\
    \verb'$\mathit{conf}_a$' & $\qquad \mathit{conf}_a$
  \end{tabular}
\end{center}
See The \TeX book, p.\ 165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, \emph{e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', 
shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et\hskip 0.1em}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.


\subsection{Most Frequently Encountered Issues}
Please kindly use the checklist below to deal with some of the most frequently encountered issues in the latex files of ECCV submissions.

\begin{itemize}
\item I have removed all \verb| \vspace| and \verb|\hspace|  commands from my paper.
\item I have not used \verb|\cite| command in the abstract.
\item I have entered a correct \verb|\titlerunning{}| command and selected a meaningful short name for the paper.
\item I have used the same name spelling in all my papers accepted to ECCV and ECCV Workshops.
\item I have added acknowledgments without a section number, e.g. using the \verb|\section*{}| command.
\item Excluding references and acknowledgments, my paper is no longer than 14 pages.
\item I have not decreased the font size of any part of the paper (except tables) to fit into 14 pages, I understand Springer editors will remove such commands.
\end{itemize}


\section{Conclusion}
The paper ends with a conclusion. 

\clearpage\mbox{}Page \thepage\ of the manuscript.
\clearpage\mbox{}Page \thepage\ of the manuscript.
\clearpage\mbox{}Page \thepage\ of the manuscript.
\clearpage\mbox{}Page \thepage\ of the manuscript.
\clearpage\mbox{}Page \thepage\ of the manuscript. This is the last page.
\par\vfill\par
Now we have reached the maximum length of an ECCV \ECCVyear{} submission (excluding references and acknowledgements).
References should start immediately after the main text, but can continue past p.\ 14 if needed. 
\clearpage  % TODO FINAL: This \clearpage needs to be removed from both review and camera-ready versions.

\section*{Acknowledgements}
Please insert your acknowledgments here.


==> sec/figures_and_tables_tex/arch_region_corresp.tex <==
\begin{figure*}[ht]
  \centering
 \includegraphics[width=\textwidth]{sec/figures_and_tables_tex/region_corresp_net.pdf}
  % \includegraphics[width=\textwidth]{sec/figures_and_tables_tex/region_corresp_net-v2.pdf}
  
  \caption{
  \red{\textbf{Appearance pointer generation.}
For each region, our framework encodes images, text descriptions, and spatial masks into modality-specific tokens using an image or text encoder. 
These tokens are processed by a correspondence transformer that fuses appearance cues with their associated masks to produce \emph{regional tokens} capturing region-specific information. 
For text-based conditioning, the correspondence transformer directly outputs a compact set of \emph{appearance pointers}. 
For image-based conditioning, however, the regional tokens tend to be numerous, as each image contributes multiple spatial tokens. 
To prevent the number of appearance pointers from scaling with the number of regions, we use a \emph{spatial aggregation transformer} that consolidates all regional tokens corresponding to the same spatial location into a single representation. 
This produces a fixed set of \emph{image appearance pointers} that remains constant regardless of how many conditioning regions are provided.}
  }
  \label{fig:arch_precisegen}
\end{figure*}

==> sec/figures_and_tables_tex/fig_attention_map.tex <==
\begin{figure}[t]
  \centering
  % \vspace{-0.05in}
  \includegraphics[width=\linewidth]{sec/figures_and_tables_tex/pdfs/Attention_maps_2.pdf}
  \vspace{-0.3in}
  \caption{\textbf{Appearance Pointer Attention Maps} (\Rone, \Rthree). 
  Each column displays region mask in row 1, attention map for image pointer ($^{I}\mathcal{AP}$) in row 2 and attention for text pointer ($^{T}\mathcal{AP}$) in row 3. 
  % Each column \textbf{(Row 1)} input spatial regions, \textbf{(Row 2)} attention for Image Pointer ($^{I}\mathcal{AP}$), and \textbf{(Row 3)} attention for Text Pointer ($^{T}\mathcal{AP}$).
  Maps are computed via cross attention between Appearance Pointer (query) and generative tokens (key). 
  Following the visualization style of Prompt-to-Prompt [Amir Hertz et. al.], we average these maps across all timesteps and visualize the top-3 PCA components along the head dimension as RGB channels (R: PC1, G: PC2, B: PC3), followed by Gaussian smoothing.
  % These maps are averaged across all times and their top-3 PCA components along the head dimension are visualized channelwise (R: PC1, G: PC2, B: PC3) followed by Gaussian Smoothing (Row 2-3) as in Prompt-To-Prompt [Amir Hertz et. al.]. 
  % We compute the average attention map by attending the appearance pointer tokens (query) to the generation tokens (key) as key during generation and then select \textbf{the top-3 principal components} across attention heads followed by gaussian smoothing as done in Prompt-To-Prompt [Amir Hertz et. al.]. 
  Appearance Pointers \textbf{points to \& delineates regions of interest} adhering to the provided region masks.
  Note \textbf{PCA orders RGB components based on maximum variance} instead of its importance.}
  \vspace{-0.25in}
  \label{fig:appearance_pointer_attention_map}
\end{figure}

==> sec/figures_and_tables_tex/fig_qual_rebuttal.tex <==
\begin{figure}[H]
  \centering
  \vspace{-0.16in}
  \includegraphics[width=\linewidth]{sec/figures_and_tables_tex/pdfs/Qual_rebuttal.pdf}
  \vspace{-0.33in}
  \caption{\textbf{Qualitative Results: Real World Pose Control \& ContextGen Comparison (\Rone, \Rtwo, \Rthree).} 
  \textbf{(top)} We can significantly alter the pose of the dog and man by changing regions.
  \textbf{(bottom)} 
  Comparison with ContextGen on placing real-world humans and objects.
  Our method enables multimodal precise spatial cues (missing in ContextGen) but falls short on facial fidelity due to limited facial data in out dataset.
  % We can hallucinate, replace humans and place objects on the table similar to ContextGen.
  % With the lack of human face data, our work struggles with real-world facial details compared to concurrent work, but ContextGen cannot provide fine-grained multimodal spatial control to repose \& edit subjects. 
  % However, the focus of our work is modular multimodal spatial control that is not addressed in prior uni-modal works. 
  % to expand it to additional modalities in the future that is not addressed in prior works.
  }
  \vspace{-0.2in}
  \label{fig:appearance_pointer_attention_map}
\end{figure}

==> sec/figures_and_tables_tex/table_backup.tex <==
\begin{figure*}
% \vspace{-0.05in}
    \centering
    \scalebox{0.85}{
\setlength{\tabcolsep}{6pt} % Default value: 6pt
\renewcommand{\arraystretch}{1} % Default value: 1
\begin{tabular}{l|cccc|cc}
    \toprule
    & \multicolumn{4}{c}{\textbf{Region}} & \multicolumn{2}{c}{\textbf{Global}}\\
    % \cline{2-5} \cline{6-7} \\
    \textbf{Method (COCO/PreciseGen Data)} & \textbf{CLIP-I}{\color{blue} $\uparrow$} &\textbf{CLIP-T}{\color{blue} $\uparrow$} & \textbf{DINO-I} {\color{blue} $\uparrow$} & \textbf{MIoU} {\color{blue} $\uparrow$} & \textbf{CLIP-T}{\color{blue} $\uparrow$} & \textbf{CLIP-IQA} {\color{blue} $\uparrow$} \\
    \midrule
    \multicolumn{7}{l}{\textbf{Text with Region Control}} \\
    \midrule
    \textbf{InstanceDiffusion~\cite{wang2024instancediffusion}} & 88.67/86.39 & 26.41/27.54 & 39.29/35.02 & 35.26/41.04 & 29.44/26.70 & 92.81/93.37 \\
    \textbf{DreamRenderer with Depth~\cite{zhou2025dreamrenderer}} & 88.51/87.75 & 26.52/28.03 & 41.30/44.20 & 32.44/33.84 & 30.16/28.43 & 92.78/93.24 \\
    \textbf{Seg2Any~\cite{zhang2025seg2any}} & 90.19/89.11 & 26.65/27.67 & 45.95/50.05 & 38.59/36.37& 30.72/29.30 & 91.89/94.59 \\
    \textbf{\coolname (Ours)} & 88.74/90.40 & 25.00/27.24 & 40.95/56.09 & 37.35/40.35 & 30.12/28.93 & 92.96/95.02 \\
    \midrule
    \multicolumn{7}{l}{\textbf{Image with Region Control (Generation w/o Background)}} \\
    \midrule
    \textbf{MSDiffusion~\cite{wang2025msdiffusion} (Bbox)} & 87.57/89.66 & 25.10/24.89 & 42.02/45.61 & 23.98/28.86 & 31.90/31.08 & 83.91/74.85 \\
    \textbf{\coolname (Ours) (Regions)} & 93.29 & 27.25 & 69.31 & 40.97  &  29.62 & 95.57 \\
    % \textbf{Flux-Kontext?~\cite{flux_kontext}} & & & & \\
    \midrule
    \multicolumn{7}{l}{\textbf{Image with Region Control with Background (Editing)}} \\
    \midrule
    \textbf{Iterative InsertAnything~\cite{song2025insert}} & 95.28/94.52 & 25.61/27.46  & 71.52/76.32 & 41.79/40.63 & 30.17/29.74 & 59.07/85.82  \\
    \textbf{\coolname (Ours)} & 93.38/94.57 & 25.40/27.66 & 60.03/74.97 & 43.84/(44.67) & 30.72/30.09 & 76.7/95.46 \\
    \midrule
    \multicolumn{7}{l}{\textbf{Multi-Modal Control (Image, Text, and Region Control)} \rahul{need to change title and numbers accordingly}} \\
    \midrule
    \textbf{\coolname w/o Spatial Aggregation Mask} & 93.38/94.57 & 25.40/27.66 & 60.03/74.97 & 43.84/(44.67) & 30.72/30.09 & 76.7/95.46 \\
    \textbf{\coolname with Spatial Aggregation Mask} & 94.52 & 27.69 & 75.11 & 45.44 & 30.03& 95.47\\
    \textbf{\coolname w/o Edge Control} & & & & & &\\
    % \textbf{\coolname (Ours)} & &  & & & & \\
    \bottomrule
\end{tabular}
}
    % \vspace{-0.3cm}
    % \end{table*}
    \captionof{table}{test
    \label{tab:metrics}}
% \vspace{-0.7cm}
\end{figure*}


==> sec/figures_and_tables_tex/table_main.tex <==
\begin{figure*}
% \vspace{-0.05in}
    \centering
    \scalebox{0.85}{
\setlength{\tabcolsep}{6pt} % Default value: 6pt
\renewcommand{\arraystretch}{1} % Default value: 1
\begin{tabular}{l|cccc|cc}
    \toprule
    & \multicolumn{4}{c}{\textbf{Region}} & \multicolumn{2}{c}{\textbf{Global}}\\
    % \cline{2-5} \cline{6-7} \\
    \textbf{Method (COCO/PreciseGen Data)} & \textbf{CLIP-I}{\color{blue} $\uparrow$} &\textbf{CLIP-T}{\color{blue} $\uparrow$} & \textbf{DINO-I} {\color{blue} $\uparrow$} & \textbf{MIoU} {\color{blue} $\uparrow$} & \textbf{CLIP-T}{\color{blue} $\uparrow$} & \textbf{CLIP-IQA} {\color{blue} $\uparrow$} \\
    \midrule
    \multicolumn{7}{l}{\textbf{Text with Region Control}} \\
    \midrule
    \textbf{InstanceDiffusion~\cite{wang2024instancediffusion}} & 88.67/86.39 & 26.41/27.54 & 39.29/35.02 & 35.26/41.04 & 29.44/26.70 & 92.81/93.37 \\
    \textbf{DreamRenderer with Depth~\cite{zhou2025dreamrenderer}} & 88.51/87.75 & 26.52/28.03 & 41.30/44.20 & 32.44/33.84 & 30.16/28.43 & 92.78/93.24 \\
    \textbf{Seg2Any~\cite{zhang2025seg2any}} & 90.19/89.11 & 26.65/27.67 & 45.95/50.05 & 38.59/36.37& 30.72/29.30 & 91.89/94.59 \\
    \textbf{\coolname (Ours)} & 88.74/90.40 & 25.00/27.24 & 40.95/56.09 & 37.35/40.35 & 30.12/28.93 & 92.96/95.02 \\
    \midrule
    \multicolumn{7}{l}{\textbf{Image with Region Control (Generation w/o Background)}} \\
    \midrule
    \textbf{MSDiffusion~\cite{wang2025msdiffusion} (Bbox)} & 87.57/89.66 & 25.10/24.89 & 42.02/45.61 & 23.98/28.86 & 31.90/31.08 & 83.91/74.85 \\
    \textbf{\coolname (Ours) (Regions)} & 93.29 & 27.25 & 69.31 & 40.97  &  29.62 & 95.57 \\
    % \textbf{Flux-Kontext?~\cite{flux_kontext}} & & & & \\
    \midrule
    \multicolumn{7}{l}{\textbf{Image with Region Control with Background (Editing)}} \\
    \midrule
    \textbf{Iterative InsertAnything~\cite{song2025insert}} & 95.28/94.52 & 25.61/27.46  & 71.52/76.32 & 41.79/40.63 & 30.17/29.74 & 59.07/85.82  \\
    \textbf{\coolname (Ours)} & 93.38/94.57 & 25.40/27.66 & 60.03/74.97 & 43.84/(44.67) & 30.72/30.09 & 76.7/95.46 \\
    \midrule
    \multicolumn{7}{l}{\textbf{Multi-Modal Control (Image, Text, and Region Control)} \rahul{need to change title and numbers accordingly}} \\
    \midrule
    \textbf{\coolname w/o Spatial Aggregation Mask} & 93.38/94.57 & 25.40/27.66 & 60.03/74.97 & 43.84/(44.67) & 30.72/30.09 & 76.7/95.46 \\
    \textbf{\coolname with Spatial Aggregation Mask} & 94.52 & 27.69 & 75.11 & 45.44 & 30.03& 95.47\\
    \textbf{\coolname w/o Edge Control} & & & & & &\\
    % \textbf{\coolname (Ours)} & &  & & & & \\
    \bottomrule
\end{tabular}
}
    % \vspace{-0.3cm}
    % \end{table*}
    \captionof{table}{test
    \label{tab:metrics}}
% \vspace{-0.7cm}
\end{figure*}


==> sec/rebuttal/01_rebuttal.tex <==


% \rahul{Some lines are repeated I need to pick more diverse reviews}
% \vspace{-4in}
We thank the reviewers for their valuable feedback \& positive comments such as \coolname ``\emph{provides valuable solution to a critical problem(...) linking multimodal cues to spatial regions in DiTs}" (\Rtwo) and that ``\emph{the results shown in the paper are visually compelling}" (\Rthree) while ``\emph{providing timely contribution that enables both text and image cues for regional control} (\Rone).
Finally, Reviewer \Rtwo{} finds our method ``\emph{a simple, multi-modality-compatible solution to DiTs’ lack of spatial control}''. 
% \coolname is the first model of its kind that enables heterogeneous spatial controls including text, image, and texture which is a hard problem. 
We resolve reviewer queries below.
% We believe this rebuttal resolves the review
% It is unfortunate that \Rone{} did not provide a clear path to improve the quality of the paper to increase its rating. 




% However, due to the lack of modular feature aggregation the model fails to preserve identity
% \todo{cover mask transformer, need for region correspondence, and mention other ablations are already in supp.}

% \srinath{Didn't multiple reviewers bring up the qualitative/visual results. Should that go first?}

% \parahead{Appearance Pointer Attention Map (\Rone, \Rthree)}
% In ~\cref{fig:appearance_pointer_attention_map} we visualize the top 3 principal components (with RGB) of the average attention map between appearance pointer tokens (query) and generation tokens (key) following Prompt-To-Prompt [A.Hertz et. al.].
% Appearance Pointers successfully localizes different objects and controls regions based on the spatial constraint during image generation.

\parahead{Quantitative Comparison (\Rone, \Rtwo)}
% \matheus{I think this should be the first point in the rebuttal.
% We should mention that our results might not be on par with recent proprietary models,
% but, to the best of our knowledge, its performance is quantitatively better than
% open source alternatives doing similar tasks (point to quantitative).
% }
% \rahul{I think we should mention that heterogeneous region control is difficult and we still beat unimodal opensource benchmarks.}
% \matheus{Very good point!}
We benchmark DreamRenderer with image + b.box + depth control where the depth is obtained by Depth-Anything on images from our dataset providing DreamRenderer* with unfair advantage.
% \matheus{briefly explain why}
DreamRenderer* fails to match our precision as it overlooks small regions and misses objects: Region (CLIP-I: 92.08 vs. \underline{93.29} (ours), CLIP-T: \underline{27.37} vs 27.25 (ours), DINO-I: 64.20 vs \underline{69.31} (ours),  MIoU: 40.11 vs \underline{40.97} (ours)) \& Global (CLIP-IQA: 89.56 vs \underline{95.57} (ours), CLIP-T: \underline{30.02} vs 29.62 (ours)). 
This 5.11-point gap is critical, as DINO-I is more sensitive to structural and identity consistency.
We are unable to compare InContext Brush as their code is not public (\Rone). 
We will cite this work.
% The marginal improvement in CLIP-T depth map contains the scene context (such as object orientation and objects in background) improving adherance to the global prompt.

\input{sec/figures_and_tables_tex/fig_qual_rebuttal}
% \todo{Visualize!!!!}

% \parahead{Model Complexity \& Ablations (\Rone{}, \Rthree{})}
% As in manu. (L:), we downsample the number of tokens to reduce the quadratic complexity and instead add contours for precise edits (ablated in tab. 1 supp.)
% Additionally, 
% We thank \Rone{}, \Rthree{} for questioning the complexity of our model.

% \matheus{We should have a sentence that directly answers the reviewer.
% Something like ``our architecture is already as simple as just using MLPs''.
% For simplicity, we might even}

\parahead{Memory Complexity (\Rone, \Rthree)} Our mask transformer architecture with \emph{2 layer self-attention blocks} (128K params. $\approx$ 500Kb) (manu. L: 296) is already as simple as using MLPs.
Self-attention in the transformer enables patches within a mask to attend to each other providing global context.
% This is analogous in memory to 2 layer Flux-Redux image projection with the only distinction that self-attention allows mask regions to attend to each other providing global context. 
Our Region Correspondence block \emph{repurposes MM-DiT (with self-attention) from FLUX-Kontext which is already compatible with DiT} with the addition of \emph{two modalities for image region pointer \& text region pointer}. 
This block has \emph{3 layers} (1200M params. $\approx$ 2.4GB in bf16) where the param. count is because of hidden dimension size D=3072 for FLUX making it wide.
% We utilize self-attention as it is proven to be more effective than cross-attention (see ~\cite{}).

\input{sec/figures_and_tables_tex/fig_attention_map}

\parahead{Time Complexity (\Rone, \Rthree)} Our module is \emph{not time-dependent} and is \emph{run only once at inference}.
Additionally, downsampling tokens in region correspondence and \emph{attending to regions separately} reduces generation overhead from $\mathbf{O(T\cdot (R\cdot N_{region})^2)}$ to $\mathbf{O(1\cdot R\cdot (N_{region} /k)^2)}$ where $N_{region}$ is tokens per region, $R$ is number of regions, $k$ is downsampling factor, \& $T$ is timesteps. 
% Our Mask Transformer are simple 2 layer self attention blocks (manu. L:) with 
% Our Region Correspondence Model borrows MM-DiT self-attention blocks from Flux Kontext that is \textbf{already compatible with the DiT} and adds two modalities the image region pointer and text region pointer ($^{R}\hat{\mathcal{P}}_i$).

\parahead{Ablations (\Rone, \Rthree)} We ablate design choices for our work in supp. Tab. 1.  
We will move these to the manuscript.
\textit{Appearance Pointer Aggregation} improves DiNO-I by 27\% improving identity preservation.  
The \textit{Region Contours} provides fine-grained control to improve MIoU by 43\%.
See supp. for more ablations.
% The rest can be deleted}adds precision to the coarse downsampled tokens in our model (improving MIoU \& DINO-I) with more ablations in the supp. material.

% Without Appearance Pointer Aggregation (Tab.1 supp.), region correspondence with self-attention to attend text, region, and image tokens that provide inferior results (lacking identity preservation) due to leakage of one region to another. 

% \parahead{Ablations (\Rone{}, \Rthree)} 



% \todo{Write}

% \parahead{Reposing \& ContextGen Visual Comparison (\Rone, \Rtwo, \Rthree)} 
% ~\cref{fig:qualitative} shows complex real-world generations with real images. 
% Additional qualitative results are in supp. (Fig.)
% comment on figure 1 teaser and defer them to supp. for more results.
% Concurrent work ContextGen preserves human faces better than our work as we lack facial training data in \coolname. 
% But ContextGen does not enable precise mask region control that enables reposing/artistic additions to the image.
% The focus of our work is to provide a modular framework to unify spatial, text, and image representation using pointers that can possible expand to more modalities in the future.
% \todo{ContextGen visual comparison and more difficult real-world results with comments about contextgen vs our work}



\parahead{Limitations (\Rtwo) \& CLIP-T performance (\Rthree)}
Following spatial control occasionally reduces adherence to global prompt resulting in lower CLIP-T scores.
We occasionally struggle with growing number of regions (supp. Fig. 2) and in preserving facial details due to limited data.

% \todo{Write!!!!}

\parahead{Mask Transformer, Learnable Tokens \& Notations (\Rthree)} The Mask Transformer pre-aligns region mask features with the image and text features that are then fused in correspondence model. 
Learnable tokens (analogous to [CLS] token) aggregate information along the R regions capturing global region context forming the Appearance Pointer ($\mathcal{AP}$). 
% After region aggregation only the learnable tokens form the Appearance Pointer ($\mathcal{AP}$).
Eqn. 5 \& 6 have a typo (thank you) where we replace ${}^{I}M_s \to {}^I\mathcal{AP}$ \& ${}^{T}M_s\to {}^T\mathcal{AP}$.
% The $^{I}M_s$ \& $^{T}M_s$ should be replaced by $^I\mathcal{AP}$ \& $^T\mathcal{AP}$ respectively in Eqn. 5 \& 6 (thank you for mentioning the typo).
The subscript in ${H}_i$ and $H_t$ are for image and text streams, respectively.
% $H_i$ and $H_t$ are height dimensions of image and text stream respectively.

\parahead{Additional Comments (\Rone, \Rtwo, \Rthree)}
We will cite MIGC++ (\Rtwo).
The lamp in the temple scene is due to global prompt "a temple ... with a street light ...." omitted for a concise subheading (\Rone). 
The teaser task is considerably challenging that includes reposing a vehicle, imagining a dog, and creating a table with the provided texture in a new environment with \emph{fine-grained} spatial control that is not possible with \emph{prior work}. 
Please see supp. Fig. 3 \& 4 for gallery of images with multi-modal spatial control.
% \todo{typos, figure comments}

% \parahead{Summary (\Rone, \Rtwo, \Rthree)}
% \coolname is a method that implements modular components to link multi-modal controls (image, text, and texture) with their spatial regions providing the flexibility to control all these modalities for generation and insertion tasks (with background). 
% Our work also proposes a \coolname-27K dataset (containing regions, texts, images, textures) and its generation pipeline that can help the community benchmark and improve multimodal generative spatial region control.






==> sec/rebuttal/Z_template.tex <==


%%%%%%%%% BODY TEXT - ENTER YOUR RESPONSE BELOW
\section{Introduction}

After receiving paper reviews, authors may optionally submit a rebuttal to address the reviewers' comments, which will be limited to a {\bf one page} PDF file.
Please follow the steps and style guidelines outlined below for submitting your author response.

The author rebuttal is optional and, following similar guidelines to previous conferences, is meant to provide you with an opportunity to rebut factual errors or to supply additional information requested by the reviewers.
It is NOT intended to add new contributions (theorems, algorithms, experiments) that were absent in the original submission and NOT specifically requested by the reviewers.
You may optionally add a figure, graph, or proof to your rebuttal to better illustrate your answer to the reviewers' comments.

Per a passed 2018 PAMI-TC motion, reviewers should refrain from requesting significant additional experiments for the rebuttal or penalize for lack of additional experiments.
Authors should refrain from including new experimental results in the rebuttal, especially when not specifically requested to do so by the reviewers.
Authors may include figures with illustrations or comparison tables of results reported in the submission/supplemental material or in other papers.

Just like the original submission, the rebuttal must maintain anonymity and cannot include external links that reveal the author identity or circumvent the length restriction.
The rebuttal must comply with this template (the use of sections is not required, though it is recommended to structure the rebuttal for ease of reading).

%-------------------------------------------------------------------------

\subsection{Response length}
Author responses must be no longer than 1 page in length including any references and figures.
Overlength responses will simply not be reviewed.
This includes responses where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.

%------------------------------------------------------------------------
\section{Formatting your Response}

{\bf Make sure to update the paper title and paper ID in the appropriate place in the tex file.}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The top margin should begin 1 inch (2.54 cm) from the top edge of the page.
The bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the page.

Please number any displayed equations.
It is important for readers to be able to refer to any particular equation.

Wherever Times is specified, Times Roman may also be used.
Main text should be in 10-point Times, single-spaced.
Section headings should be in 10 or 12 point Times.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Figure and table captions should be 9-point Roman type as in \cref{fig:onecol}.


List and number all bibliographical references in 9-point Times, single-spaced,
at the end of your response.
When referenced in the text, enclose the citation number in square brackets, for example~\cite{Alpher05}.
Where appropriate, include the name(s) of editors of referenced books.

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{0.5in} \rule{0.9\linewidth}{0pt}}
  %\includegraphics[width=0.8\linewidth]{egfigure.eps}
   \caption{Example of caption.  It is set in Roman so that mathematics
   (always set in Roman: $B \sin A = A \sin B$) may be included without an
   ugly clash.}
   \label{fig:onecol}
\end{figure}

To avoid ambiguities, it is best if the numbering for equations, figures, tables, and references in the author response does not overlap with that in the main paper (the reviewer may wonder if you talk about \cref{fig:onecol} in the author response or in the paper).
See \LaTeX\ template for a workaround.

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
Please ensure that any point you wish to make is resolvable in a printed copy of the response.
Resize fonts in figures to match the font in the body text, and choose line widths which render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your response in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it is almost always best to use \verb+\includegraphics+, and to specify the  figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}

%%%%%%%%% REFERENCES
{
    \small
    \bibliographystyle{ieeenat_fullname}
    \bibliography{main}
}

